On Improving the Cohesiveness of Graphs by Merging Nodes: Formulation, Analysis, and Algorithms

Graphs are a powerful mathematical model, and they are used to represent real-world structures in various fields. In many applications, real-world structures with high connectivity and robustness are preferable. For enhancing the connectivity and robustness of graphs, two operations, adding edges and anchoring nodes, have been extensively studied. However, merging nodes, which is a realistic operation in many scenarios (e.g., bus station reorganization, multiple team formation), has been overlooked. In this work, we study the problem of improving graph cohesiveness by merging nodes. First, we formulate the problem mathematically using the size of the $k$-truss, for a given $k$, as the objective. Then, we prove the NP-hardness and non-modularity of the problem. After that, we develop BATMAN, a fast and effective algorithm for choosing sets of nodes to be merged, based on our theoretical findings and empirical observations. Lastly, we demonstrate the superiority of BATMAN over several baselines, in terms of speed and effectiveness, through extensive experiments on fourteen real-world graphs.

==> FIG/bus_visual.tex <==
\begin{figure*}[t!]    
    \centering
    % \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{FIG/bus_visual/kuopio.pdf}
    %      \caption{kuopio}         
    %  \end{subfigure}
    %  \hfill
    %  \begin{subfigure}[b]{0.32\textwidth}
    %      \centering
    %      \includegraphics[width=\textwidth]{FIG/bus_visual/nantes.pdf}
    %      \caption{nantes}         
    %  \end{subfigure}
    %  \hfill        
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{FIG/bus_visual/helsinki.pdf}
         \caption{helsinki}         
     \end{subfigure}
     \hfill       
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{FIG/bus_visual/rome.pdf}
         \caption{rome}         
     \end{subfigure}
     \hfill           
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{FIG/bus_visual/brisbane.pdf}
         \caption{brisbane}         
     \end{subfigure}
     \hfill         
     \begin{subfigure}[b]{0.24\textwidth}
         \centering
         \includegraphics[width=\textwidth]{FIG/bus_visual/paris.pdf}
         \caption{paris}         
     \end{subfigure}
    \caption{\crr{The results of the proposed method \bmshort in the additional experiments on real-world bus station datasets.}
    \label{fig:bus_visual}}
    \vspace{-1mm}
\end{figure*}

==> FIG/different_b.tex <==
\begin{figure}[t!]
    \centering
    % \vspace{-5mm}
    % \includegraphics[width=0.9\linewidth]
    % {FIG/k_low_high_avg.pdf}
    % \includegraphics[height=0.35\linewidth, width=0.7\linewidth]
    \includegraphics[height=0.35\linewidth]
    {FIG/b_avg_0801.pdf}
    \includegraphics[height=0.35\linewidth]{FIG/legend2.pdf}
    \caption{The results with each algorithm with different budget $b$.
    The proposed method and its variants consistently outperform the baseline methods.    
    }
    \label{fig:b_avg}
\end{figure}

==> FIG/different_k.tex <==
\begin{figure}[t!]
    \centering
    % \vspace{-5mm}
    % \includegraphics[width=0.9\linewidth]
    % {FIG/k_low_high_avg.pdf}
    % \includegraphics[height=0.35\linewidth, width=0.7\linewidth]
    \includegraphics[height=0.35\linewidth]
    {FIG/k_low_high_avg.pdf}
    \includegraphics[height=0.35\linewidth]
    {FIG/b_avg_0801.pdf}
    \includegraphics[height=0.35\linewidth]{FIG/legend2.pdf}
    \caption{The average performance of each algorithm overall datasets when the trussness $k$ varies.
    The proposed method (BM) and its variants (EQ, II, and IO) outperform the baseline methods (NT, NE, and RD) for both low and high $k$ values.}    
    % Notably, when $k$ is low, inside-inside mergers perform much better than inside-outside mergers w.r.t the increase in the truss size;
    % but when $k$ is large, this superiority is reversed, and considering both cases shows higher necessity.
    % }
    \label{fig:k_avg}
\end{figure}

==> FIG/heu_node_comp.tex <==
\begin{figure}[t!]
    \centering
    % \vspace{-5mm}
    \includegraphics[height=0.36\linewidth]{FIG/heu_node_io.pdf}    
    \includegraphics[height=0.36\linewidth]{FIG/heu_node_ii.pdf}   
    \caption{Comparing different heuristics for choosing inside nodes. 
    Left: choosing inside nodes for inside-outside mergers.
    Right: choosing inside nodes for inside-inside mergers.
    }
    \label{fig:heu_node_comp}
\end{figure}


==> FIG/heu_pair_comp.tex <==
\begin{figure}[t!]
    \centering
    % \vspace{-5mm}
    \includegraphics[height=0.36\linewidth]{FIG/heu_pair_io.pdf}    
    \includegraphics[height=0.36\linewidth]{FIG/heu_pair_ii.pdf}   
    \caption{Comparing different heuristics for choosing mergers.
    Left: choosing inside-outside mergers.
    Right: choosing inside-inside mergers.
    }
    \label{fig:heu_pair_comp}
\end{figure}


==> TAB/effectiveness_merging.tex <==
\begingroup
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.8}
\begin{table}[t!]
    \vspace{-4mm}
	\begin{center}
		\caption{Merging nodes is much more effective than adding edges in enhancing graph cohesiveness and robustness. For each measure, we report the change of it when we do 10 times of merging nodes or adding edges, over five independent trials, with the original value below the measure name.
        For each measure, the first result of merging nodes that is better than adding 10 edges is marked in bold and underlined.
        \red{See Section~\ref{sec:exp} for the details.}
        }
		\label{tab:effective_merging}
			\resizebox{\linewidth}{!}{%
			\begin{tabular}{ c | c | *{10}{c}}
				\toprule
				measure & \# operations & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 \\
				\midrule                
                VB & merging & 83.1 & \underline{\textbf{79.2}} & 75.5 & 71.9 & 68.4 & 65.4 & 62.5 & 59.9 & 57.5 & 55.4 \\
                87.3 & adding & 86.2 & 85.4 & 84.7 & 84.1 & 83.5 & 83.0 & 82.5 & 82.1 & 81.6 & 81.2 \\
                \midrule
                EB & merging & 23.3 & 21.6 & \underline{\textbf{20.0}} & 18.6 & 17.4 & 16.3 & 15.2 & 14.2 & 13.3 & 12.4 \\
                25.3 & adding & 24.6 & 24.1 & 23.6 & 23.2 & 22.8 & 22.5 & 22.1 & 21.7 & 21.4 & 21.1 \\
                \midrule
                ER & merging & 714.8 & 633.0 & \underline{\textbf{570.2}} & 515.7 & 468.5 & 427.0 & 389.3 & 355.2 & 325.1 & 297.5 \\
                834.8 & adding & 776.1 & 739.5 & 712.3 & 689.9 & 671.1 & 654.0 & 639.7 & 626.0 & 613.1 & 601.3 \\
                \midrule
                NC & merging & 3.1 & 3.6 & \underline{\textbf{4.0}} & 4.3 & 4.7 & 5.0 & 5.4 & 5.7 & 6.0 & 6.2 \\
                2.7 & adding & 2.8 & 2.9 & 3.0 & 3.1 & 3.2 & 3.4 & 3.5 & 3.6 & 3.7 & 3.9 \\
                \midrule
                SG & merging & 3.1 & 3.7 & \underline{\textbf{4.3}} & 4.7 & 5.2 & 5.5 & 5.9 & 6.2 & 6.5 & 6.8 \\
                2.3 & adding & 2.5 & 2.7 & 2.9 & 3.1 & 3.2 & 3.4 & 3.6 & 3.7 & 3.9 & 4.0 \\
				\bottomrule %
			\end{tabular}
		}
	\end{center}
\end{table}
\endgroup

% ('average_edge_betweenness', 'add') [25.298 24.646 24.122 23.642 23.228 22.83  22.45  22.086 21.74  21.408
%  21.084]
% ('average_edge_betweenness', 'merge') [25.298 23.322 21.554 20.042 18.646 17.388 16.254 15.19  14.186 13.25
%  12.366]
% ('average_vertex_betweenness', 'add') [87.302 86.206 85.402 84.666 84.09  83.538 83.014 82.526 82.064 81.624
%  81.184]
% ('average_vertex_betweenness', 'merge') [87.302 83.104 79.158 75.52  71.892 68.418 65.416 62.548 59.87  57.512
%  55.376]
% ('effective_resistance', 'add') [834.798 776.064 739.498 712.288 689.918 671.062 654.018 639.65  625.952
%  613.078 601.25 ]
% ('effective_resistance', 'merge') [834.798 714.812 633.    570.15  515.702 468.518 427.034 389.268 355.178
%  325.092 297.54 ]
% ('natural_connectivity', 'add') [2.658 2.766 2.878 2.996 3.114 3.238 3.366 3.488 3.612 3.742 3.88 ]
% ('natural_connectivity', 'merge') [2.658 3.114 3.566 3.972 4.348 4.708 5.044 5.378 5.69  5.97  6.248]
% ('spectral_gap', 'add') [2.278 2.544 2.716 2.886 3.072 3.242 3.41  3.572 3.73  3.884 4.04 ]
% ('spectral_gap', 'merge') [2.278 3.056 3.736 4.288 4.746 5.178 5.536 5.914 6.204 6.498 6.79 ]


==> TAB/main_results.tex <==
\begingroup
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{0.8}
\begin{table*}[t!]
	\begin{center}
		\caption{The \textit{email} dataset is the only one among all the used datasets on which we can check for each possible   pair in each round and finish the whole process in 48 hours. The results are: 237, 989, 1523, 1482, for $k = 5, 10, 15, 20$, respectively.}
		\label{tab:main_results}
			\resizebox{\linewidth}{!}{%
			\begin{tabular}{l|c|*{6}{c}|*{6}{c}|*{6}{c}}
                \toprule
                \multicolumn{2}{c|}{$n_C$} &
                \multicolumn{6}{c|}{1} &
                \multicolumn{6}{c|}{10} &
                \multicolumn{6}{c}{100}
                % \multicolumn{6}{c|}{1000} &
                \\
                \midrule
                % \textbf{Dataset}
                & $k$ &
                RD & NE & NT & II & IO & BM &
                RD & NE & NT & II & IO & BM & 
                RD & NE & NT & II & IO & BM
                % RD &     
                \\
                \midrule                    
                % \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{EM}}} & 5\\
                \multirow{4}{*}{EM} & 5\\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{FB} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{ER} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{BK} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{RL} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{EP} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{HP} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{SD} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{SC} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{GW} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{TT} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{SF} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{YT} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule
                \multirow{4}{*}{WT} & 5 \\
                & 10 \\
                & 15 \\
                & 20 \\                
                \midrule           
                \multicolumn{2}{c|}{avg. result}
                \\
                \multicolumn{2}{c|}{avg. rank}
                \\
                \multicolumn{2}{c|}{avg. runtime} \\
                \bottomrule
			\end{tabular}
		}
	\end{center}
\end{table*}
\endgroup

==> res_heu_exp.tex <==
\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 21 & 150 & 331 & 255 \\
			& & IN & 21 & 150 & 331 & 255 \\
			& & RD & 18.7 & 97.0 & 289.3 & 255.0 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 21 & 150 & 196 & 255\\
			& & NN & 21 & 27 & 195 & 0 \\
			& & RD & 7.0 & 39.3 & 124.0 & 133.0 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 46 & 192 & 385 & 227 \\
			& & IN & 47 & 200 & 381 & 227 \\
			& & RD & 27.7 & 127.3 & 320.7 & 227.0 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 30 & 175 & 255 & 227 \\
			& & AE & 18 & 150 & 291 & 206 \\
			& & RD & 14.0 & 78.0 & 181.7 & 129.0 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{email}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_email}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 12 & 128 & 142 & 227 \\
			& & IN & 5 & 93 & 54 & 61 \\
			& & RD & 8.3 & 100.0 & 105.0 & 188.7 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 12 & 128 & 128 & 165\\
			& & NN & 0 & 16 & 29 & 151 \\
			& & RD & 3.0 & 7.0 & 48.7 & 85.7 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 21 & 100 & 151 & 171 \\
			& & IN & 7 & 17 & 24 & 18 \\
			& & RD & 12.3 & 73.7 & 92.3 & 116.7 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 17 & 46 & 151 & 169 \\
			& & AE & 15 & 74 & 50 & 72 \\
			& & RD & 7.0 & 22.3 & 36.0 & 14.3 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{facebook}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_facebook}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 79 & 100 & 204 & 195 \\
			& & IN & 79 & 100 & 126 & 151 \\
			& & RD & 34.0 & 77.0 & 181.7 & 150.7 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 79 & 72 & 204 & 150\\
			& & NN & 62 & 24 & 76 & 88 \\
			& & RD & 38.7 & 34.7 & 36.3 & 72.3 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 452 & 161 & 238 & 181 \\
			& & IN & 452 & 161 & 72 & 37 \\
			& & RD & 54.0 & 81.7 & 159.3 & 113.7 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 452 & 161 & 136 & 71 \\
			& & AE & 452 & 161 & 136 & 58 \\
			& & RD & 130.3 & 51.3 & 36.3 & 85.0 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{brightkite}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_brightkite}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 104 & 145 & 461 & 1058 \\
			& & IN & 104 & 149 & 456 & 1058 \\
			& & RD & 13.3 & 126.0 & 413.0 & 971.0 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 104 & 122 & 364 & 806\\
			& & NN & 10 & 82 & 101 & 666 \\
			& & RD & 10.7 & 53.3 & 162.7 & 659.7 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 139 & 315 & 445 & 1224 \\
			& & IN & 97 & 315 & 429 & 1224 \\
			& & RD & 10.3 & 131.0 & 348.7 & 992.0 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 139 & 315 & 330 & 1115 \\
			& & AE & 57 & 315 & 330 & 1115 \\
			& & RD & 59.0 & 128.7 & 215.0 & 606.3 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{enron}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_enron}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 71 & 441 & 409 & 430 \\
			& & IN & 73 & 441 & 409 & 430 \\
			& & RD & 30.0 & 272.0 & 321.3 & 428.7 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 71 & 441 & 409 & 430\\
			& & NN & 19 & 61 & 23 & 0 \\
			& & RD & 10.7 & 182.0 & 15.7 & 198.7 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 267 & 531 & 328 & 407 \\
			& & IN & 227 & 556 & 231 & 115 \\
			& & RD & 34.0 & 156.7 & 219.7 & 399.3 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 267 & 531 & 312 & 108 \\
			& & AE & 267 & 531 & 328 & 115 \\
			& & RD & 22.3 & 108.0 & 22.3 & 21.0 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{hepph}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_hepph}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 102 & 550 & 770 & 1069 \\
			& & IN & 102 & 550 & 770 & 1205 \\
			& & RD & 45.0 & 385.3 & 705.7 & 1081.3 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 102 & 550 & 770 & 1054\\
			& & NN & 49 & 243 & 457 & 445 \\
			& & RD & 39.3 & 237.3 & 417.0 & 487.7 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 1177 & 1113 & 1105 & 1067 \\
			& & IN & 1177 & 1113 & 1129 & 914 \\
			& & RD & 117.7 & 543.3 & 725.7 & 858.3 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 1177 & 1113 & 1105 & 958 \\
			& & AE & 1093 & 1113 & 1105 & 841 \\
			& & RD & 333.0 & 585.7 & 590.7 & 778.0 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{epinions}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_epinions}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 62 & 115 & 246 & 260 \\
			& & IN & 62 & 115 & 246 & 311 \\
			& & RD & 28.3 & 82.0 & 185.3 & 264.0 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 59 & 89 & 246 & 186\\
			& & NN & 20 & 57 & 90 & 165 \\
			& & RD & 33.3 & 76.0 & 81.0 & 113.3 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 265 & 259 & 255 & 236 \\
			& & IN & 265 & 248 & 410 & 287 \\
			& & RD & 29.0 & 123.3 & 228.7 & 241.7 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 265 & 259 & 244 & 236 \\
			& & AE & 224 & 259 & 196 & 236 \\
			& & RD & 79.7 & 68.7 & 107.3 & 83.0 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{relato}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_relato}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 621 & 171 & 192 & 154 \\
			& & IN & 621 & 179 & 189 & 154 \\
			& & RD & 329.3 & 166.0 & 176.3 & 142.0 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 621 & 150 & 185 & 135\\
			& & NN & 237 & 89 & 171 & 83 \\
			& & RD & 201.0 & 64.0 & 81.3 & 81.7 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 2737 & 186 & 233 & 136 \\
			& & IN & 2737 & 177 & 233 & 151 \\
			& & RD & 495.7 & 136.3 & 173.3 & 124.7 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 2737 & 186 & 136 & 124 \\
			& & AE & 2737 & 153 & 233 & 136 \\
			& & RD & 918.3 & 65.7 & 120.3 & 68.7 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{slashdot}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_slashdot}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 67 & 259 & 287 & 859 \\
			& & IN & 67 & 259 & 287 & 722 \\
			& & RD & 32.7 & 171.3 & 212.0 & 790.3 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 67 & 240 & 249 & 859\\
			& & NN & 57 & 259 & 249 & 216 \\
			& & RD & 11.3 & 65.3 & 72.7 & 72.0 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 525 & 973 & 634 & 809 \\
			& & IN & 525 & 973 & 634 & 414 \\
			& & RD & 60.0 & 226.0 & 231.7 & 400.7 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 525 & 973 & 463 & 709 \\
			& & AE & 525 & 973 & 634 & 414 \\
			& & RD & 98.3 & 382.3 & 129.0 & 231.7 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{syracuse}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_syracuse}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 334 & 496 & 376 & 757 \\
			& & IN & 334 & 496 & 470 & 757 \\
			& & RD & 28.0 & 147.0 & 297.3 & 735.0 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 334 & 427 & 376 & 757\\
			& & NN & 63 & 161 & 270 & 593 \\
			& & RD & 42.7 & 133.3 & 219.7 & 233.7 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 2802 & 853 & 601 & 779 \\
			& & IN & 2802 & 853 & 601 & 676 \\
			& & RD & 28.3 & 144.0 & 319.3 & 574.3 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 2802 & 810 & 601 & 529 \\
			& & AE & 2802 & 853 & 437 & 529 \\
			& & RD & 460.7 & 399.0 & 207.0 & 273.7 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{gowalla}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_gowalla}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 214 & 345 & 443 & 540 \\
			& & IN & 214 & 345 & 520 & 483 \\
			& & RD & 12.0 & 84.7 & 193.0 & 340.0 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 214 & 345 & 306 & 327\\
			& & NN & 147 & 251 & 197 & 167 \\
			& & RD & 18.3 & 84.0 & 147.7 & 113.7 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 632 & 955 & 815 & 787 \\
			& & IN & 632 & 955 & 815 & 787 \\
			& & RD & 12.0 & 62.7 & 146.7 & 280.3 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 632 & 955 & 815 & 414 \\
			& & AE & 632 & 955 & 815 & 414 \\
			& & RD & 62.0 & 332.3 & 355.3 & 315.7 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{twitter}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_twitter}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 1212 & 1853 & 4036 & 704 \\
			& & IN & 423 & 1853 & 4036 & 676 \\
			& & RD & 680.3 & 1363.7 & 2435.3 & 260.3 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 1212 & 1853 & 4036 & 704\\
			& & NN & 0 & 1165 & 0 & 0 \\
			& & RD & 344.3 & 215.7 & 462.7 & 215.7 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 2407 & 4879 & 4054 & 648 \\
			& & IN & 1454 & 2868 & 4054 & 144 \\
			& & RD & 244.7 & 896.0 & 607.7 & 55.0 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 2407 & 4879 & 4054 & 59 \\
			& & AE & 1826 & 2868 & 4054 & 14 \\
			& & RD & 317.3 & 1355.0 & 40.7 & 0.0 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{stanford}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_stanford}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 854 & 995 & 973 & 2964 \\
			& & IN & 854 & 995 & 887 & 2964 \\
			& & RD & 394.7 & 669.0 & 942.7 & 2929.3 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 854 & 995 & 973 & 2809\\
			& & NN & 54 & 512 & 724 & 1902 \\
			& & RD & 185.3 & 395.7 & 430.0 & 2151.3 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 5363 & 2145 & 952 & 2853 \\
			& & IN & 5363 & 2145 & 821 & 2853 \\
			& & RD & 239.0 & 688.0 & 808.7 & 2771.0 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 5363 & 2145 & 952 & 2813 \\
			& & AE & 4447 & 2137 & 949 & 2813 \\
			& & RD & 923.7 & 814.3 & 458.7 & 1677.0 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{youtube}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_youtube}
	\end{table*}
	\begin{table*}[h!]
		\centering
		\begin{tabular}{|c|c|c|c|c|c|c|}
			\hline
			IOMs/IIMs & nodes/pairs & heuristic & $k = 5$ & $k = 10$ & $k = 15$ & $k = 20$ \\
			\hline
			\multirow{6}{*}{IOMs}
			& \multirow{3}{*}{node-heuristics} & IP & 778 & 1595 & 930 & 344 \\
			& & IN & 778 & 1595 & 930 & 687 \\
			& & RD & 84.0 & 701.7 & 553.0 & 551.7 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 117 & 1595 & 930 & 317\\
			& & NN & 73 & 118 & 194 & 287 \\
			& & RD & 207.3 & 193.0 & 166.3 & 221.7 \\
			\hline
			\multirow{6}{*}{IIMs}
			& \multirow{3}{*}{node-heuristics} & IP & 30577 & 2687 & 1025 & 287 \\
			& & IN & 30577 & 2121 & 1144 & 954 \\
			& & RD & 121.0 & 687.3 & 555.0 & 615.3 \\
			\cline{2-7}
			& \multirow{3}{*}{pair-heuristics} & SE & 30577 & 2687 & 1025 & 214 \\
			& & AE & 30577 & 1570 & 1025 & 210 \\
			& & RD & 2892.0 & 1123.0 & 204.3 & 204.7 \\
			\hline
		\end{tabular}
		\caption{The full results of the heuristics experiments on \textit{wikitalk}.
			For each algorithm, each considered $k$ value, we report the performance of each considered node-heuristic and pair-heuristic.}
		\label{tab:heu_wikitalk}
	\end{table*}	

==> res_sampling_exp.tex <==
\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/email-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/email-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/email-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/email-20.pdf}
		\caption{The full results of the sampling experiments on \textit{email}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_email}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/facebook-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/facebook-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/facebook-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/facebook-20.pdf}
		\caption{The full results of the sampling experiments on \textit{facebook}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_facebook}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/brightkite-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/brightkite-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/brightkite-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/brightkite-20.pdf}
		\caption{The full results of the sampling experiments on \textit{brightkite}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_brightkite}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/enron-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/enron-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/enron-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/enron-20.pdf}
		\caption{The full results of the sampling experiments on \textit{enron}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_enron}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/hepph-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/hepph-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/hepph-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/hepph-20.pdf}
		\caption{The full results of the sampling experiments on \textit{hepph}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_hepph}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/epinions-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/epinions-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/epinions-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/epinions-20.pdf}
		\caption{The full results of the sampling experiments on \textit{epinions}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_epinions}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/relato-business-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/relato-business-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/relato-business-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/relato-business-20.pdf}
		\caption{The full results of the sampling experiments on \textit{relato}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_relato}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/slashdot0811-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/slashdot0811-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/slashdot0811-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/slashdot0811-20.pdf}
		\caption{The full results of the sampling experiments on \textit{slashdot}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_slashdot}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/syracuse56-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/syracuse56-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/syracuse56-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/syracuse56-20.pdf}
		\caption{The full results of the sampling experiments on \textit{syracuse}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_syracuse}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/gowalla-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/gowalla-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/gowalla-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/gowalla-20.pdf}
		\caption{The full results of the sampling experiments on \textit{gowalla}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_gowalla}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/twitter-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/twitter-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/twitter-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/twitter-20.pdf}
		\caption{The full results of the sampling experiments on \textit{twitter}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_twitter}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/stanford-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/stanford-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/stanford-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/stanford-20.pdf}
		\caption{The full results of the sampling experiments on \textit{stanford}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_stanford}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/youtube-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/youtube-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/youtube-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/youtube-20.pdf}
		\caption{The full results of the sampling experiments on \textit{youtube}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_youtube}
	\end{figure}
	
	\begin{figure}[h!]
		\centering
		\includegraphics[width=0.49\linewidth]{mean_std/wikitalk-5.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/wikitalk-10.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/wikitalk-15.pdf}
		\includegraphics[width=0.49\linewidth]{mean_std/wikitalk-20.pdf}
		\caption{The full results of the sampling experiments on \textit{wikitalk}.
			For each considered $k$ value and each case, we report the best performance among the first $x$ sampled mergers.}
		\label{fig:sampl_wikitalk}
	\end{figure}

==> tbl_main_exps.tex <==
\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (190, 0.163258) & (588, 0.395745) & (1303, 0.452645) & (1527, 0.373819) \\
        & 2 & (194, 0.297094) & (844, 0.630798) & (1376, 0.682457) & (1528, 0.434685) \\
        & 5 & (200, 0.433535) & (953, 0.704848) & (1344, 0.748737) & (1445, 0.441133) \\
        & 10 & (212, 0.536766) & (974, 0.868098) & (1343, 0.780103) & (1634, 0.503709) \\
        & 15 & (215, 0.753264) & (947, 1.10923) & (1366, 1.040943) & (1634, 0.580716) \\
        & 20 & (215, 0.939869) & (947, 1.321407) & (1278, 1.090379) & (1201, 0.571081) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (194, 0.282179) & (844, 0.611814) & (1376, 0.671509) & (1528, 0.423497) \\
        & 5 & (206, 0.349339) & (895, 0.661047) & (1304, 0.698516) & (1487, 0.456046) \\
        & 10 & (213, 0.552619) & (896, 0.864929) & (1458, 0.778773) & (1124, 0.480327) \\
        & 15 & (207, 0.691299) & (911, 1.08249) & (1406, 0.950659) & (1159, 0.512248) \\
        & 20 & (221, 0.916641) & (974, 1.288419) & (1379, 1.12371) & (1159, 0.565624) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (190, 0.138759) & (908, 0.306687) & (1303, 0.411716) & (774, 0.333101) \\
        & 2 & (204, 0.210995) & (908, 0.383291) & (1408, 0.472175) & (757, 0.343574) \\
        & 5 & (211, 0.315223) & (896, 0.516913) & (1348, 0.546718) & (1178, 0.374554) \\
        & 10 & (214, 0.484388) & (978, 0.681726) & (1435, 0.634548) & (754, 0.400293) \\
        & 15 & (213, 0.687604) & (947, 0.908359) & (1448, 0.813922) & (820, 0.470702) \\
        & 20 & (225, 0.839121) & (947, 1.11379) & (1256, 0.883392) & (820, 0.499459) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (139, 0.145697) & (588, 0.35929) & (1417, 0.416889) & (1527, 0.36234) \\
        & 2 & (138, 0.210198) & (636, 0.430234) & (1290, 0.491398) & (1238, 0.391185) \\
        & 5 & (138, 0.303721) & (588, 0.563956) & (1411, 0.578495) & (1099, 0.407051) \\
        & 10 & (145, 0.45026) & (697, 0.731267) & (1320, 0.722222) & (1634, 0.463949) \\
        & 15 & (145, 0.620213) & (641, 0.958933) & (1452, 0.844707) & (1657, 0.520014) \\
        & 20 & (145, 0.799318) & (643, 1.167234) & (1452, 0.991405) & (1608, 0.574232) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (73, 1.316854) & (428, 1.131434) & (833, 0.762351) & (626, 0.377389) \\
        & 2 & (72, 2.450766) & (504, 2.046731) & (1072, 1.327413) & (796, 0.54811) \\
        & 5 & (81, 4.92864) & (465, 4.243704) & (1135, 2.765242) & (1140, 1.070902) \\
        & 10 & (101, 7.167055) & (587, 6.50248) & (1089, 4.260347) & (1153, 1.559173) \\
        & 15 & (109, 7.344824) & (590, 6.496875) & (1114, 4.242718) & (1129, 1.541246) \\
        & 20 & (112, 7.488949) & (595, 6.70923) & (1287, 4.406364) & (1148, 1.600867) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (93, 0.074646) & (263, 0.130554) & (394, 0.190378) & (1137, 0.209669) \\
        & 2 & (93, 0.104544) & (263, 0.168751) & (394, 0.221188) & (1137, 0.21616) \\
        & 5 & (93, 0.201608) & (263, 0.289639) & (394, 0.31141) & (1137, 0.249993) \\
        & 10 & (129, 0.353582) & (433, 0.479871) & (888, 0.464709) & (1084, 0.300897) \\
        & 15 & (93, 0.511208) & (263, 0.682291) & (394, 0.580377) & (1137, 0.359938) \\
        & 20 & (93, 0.660565) & (263, 0.875819) & (394, 0.736546) & (1137, 0.39993) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (35, 0.09364) & (42, 0.202609) & (174, 0.277664) & (351, 0.30549) \\
        & 2 & (23, 0.124586) & (219, 0.251621) & (313, 0.308926) & (343, 0.307641) \\
        & 5 & (39, 0.194363) & (264, 0.309078) & (619, 0.360495) & (376, 0.324811) \\
        & 10 & (66, 0.391954) & (261, 0.557491) & (652, 0.526545) & (654, 0.404832) \\
        & 15 & (56, 0.514945) & (479, 0.710561) & (660, 0.631788) & (749, 0.446687) \\
        & 20 & (66, 0.695103) & (401, 0.935773) & (817, 0.815195) & (662, 0.491332) \\
        \hline
    \end{tabular}		
    \caption{The full results of the main experiments on \textit{email}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_email}
\end{table*}

\begin{table*}[h!]
    \centering
        \begin{tabular}{|c|c|c|c|c|c|}
            \hline
            algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
            \hline
            \multirow{6}{*}{BM}
            & 1 & (149, 0.506361) & (462, 0.948327) & (505, 1.133406) & (675, 1.171536) \\
            & 2 & (152, 1.02818) & (620, 1.508909) & (505, 1.773869) & (1095, 1.66875) \\
            & 5 & (158, 1.483856) & (640, 1.972026) & (631, 2.177783) & (1029, 2.040044) \\
            & 10 & (163, 2.351635) & (675, 2.764291) & (678, 2.927482) & (1093, 2.70812) \\
            & 15 & (177, 3.252112) & (675, 3.850927) & (636, 3.978673) & (1124, 3.711568) \\
            & 20 & (172, 4.169596) & (678, 4.697119) & (678, 4.983967) & (1099, 4.534922) \\
            \hline
            \multirow{6}{*}{EQ}
            & 1 & N/A & N/A & N/A & N/A \\
            & 2 & (152, 0.987369) & (620, 1.519664) & (505, 1.732861) & (1095, 1.669056) \\
            & 5 & (158, 1.337278) & (652, 1.808965) & (513, 2.116939) & (1076, 1.996077) \\
            & 10 & (164, 2.316492) & (675, 2.789305) & (617, 2.940854) & (1176, 2.733471) \\
            & 15 & (164, 3.114176) & (682, 3.624242) & (617, 3.789719) & (1135, 3.48443) \\
            & 20 & (171, 4.126044) & (678, 4.729749) & (678, 4.77951) & (1075, 4.421955) \\
            \hline
            \multirow{6}{*}{II}
            & 1 & (149, 0.463815) & (490, 0.796277) & (505, 1.034633) & (675, 1.115816) \\
            & 2 & (149, 0.820292) & (556, 1.177575) & (612, 1.378685) & (662, 1.40776) \\
            & 5 & (154, 1.353022) & (550, 1.731343) & (617, 1.878777) & (797, 1.890962) \\
            & 10 & (171, 2.127139) & (627, 2.483068) & (678, 2.662917) & (877, 2.489292) \\
            & 15 & (185, 3.103649) & (633, 3.549826) & (678, 3.586211) & (847, 3.418032) \\
            & 20 & (185, 4.020618) & (616, 4.406482) & (678, 4.429359) & (896, 4.202753) \\
            \hline
            \multirow{6}{*}{IO}
            & 1 & (70, 0.485909) & (462, 0.868455) & (393, 1.137245) & (981, 1.218973) \\
            & 2 & (84, 0.825116) & (531, 1.240481) & (393, 1.477159) & (1141, 1.487601) \\
            & 5 & (89, 1.337836) & (653, 1.739939) & (387, 1.996417) & (1266, 1.920456) \\
            & 10 & (89, 2.119162) & (654, 2.572274) & (352, 2.759679) & (1158, 2.568547) \\
            & 15 & (90, 3.014986) & (672, 3.503828) & (411, 3.686824) & (1226, 3.380297) \\
            & 20 & (90, 3.88141) & (657, 4.368629) & (349, 4.635049) & (1200, 4.090064) \\
            \hline
            \multirow{6}{*}{NT}
            & 1 & (25, 4.802132) & (185, 4.553131) & (165, 4.410222) & (212, 4.128859) \\
            & 2 & (25, 8.323137) & (265, 8.190111) & (175, 7.638757) & (241, 6.939943) \\
            & 5 & (20, 17.131463) & (276, 16.749262) & (232, 15.494895) & (264, 14.106341) \\
            & 10 & (20, 27.410854) & (283, 27.03053) & (264, 24.976688) & (289, 22.699999) \\
            & 15 & (24, 27.212796) & (273, 26.827285) & (296, 24.811599) & (301, 22.458058) \\
            & 20 & (27, 27.993103) & (219, 27.642417) & (292, 25.626299) & (310, 23.035773) \\
            \hline
            \multirow{6}{*}{NE}
            & 1 & (9, 0.483263) & (0, 0.610785) & (0, 0.757779) & (0, 0.890101) \\
            & 2 & (9, 0.629466) & (0, 0.787201) & (0, 0.907253) & (0, 1.020575) \\
            & 5 & (9, 1.168563) & (0, 1.28736) & (0, 1.409836) & (0, 1.496966) \\
            & 10 & (16, 1.890344) & (0, 2.065769) & (0, 2.246718) & (0, 2.158495) \\
            & 15 & (9, 2.793643) & (0, 2.996425) & (0, 3.136047) & (0, 3.003932) \\
            & 20 & (9, 3.632236) & (0, 3.903284) & (0, 3.904875) & (0, 3.791944) \\
            \hline
            \multirow{6}{*}{RD}
            & 1 & (-7, 0.478493) & (-1, 0.722488) & (-14, 0.951511) & (-157, 1.147531) \\
            & 2 & (1, 0.645246) & (10, 0.931899) & (11, 1.160903) & (5, 1.293247) \\
            & 5 & (1, 1.021822) & (23, 1.284559) & (9, 1.480335) & (38, 1.562286) \\
            & 10 & (14, 1.992733) & (32, 2.313069) & (77, 2.51362) & (86, 2.488989) \\
            & 15 & (12, 2.675058) & (34, 3.037993) & (36, 3.234321) & (46, 3.125762) \\
            & 20 & (10, 3.640068) & (117, 4.074742) & (115, 4.248889) & (49, 4.021556) \\
            \hline
        \end{tabular}			
    \caption{The full results of the main experiments on \textit{facebook}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_facebook}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (2660, 7.633889) & (759, 4.289924) & (606, 3.520721) & (738, 3.435266) \\
        & 2 & (2660, 11.775407) & (759, 5.206878) & (635, 3.837289) & (753, 3.84938) \\
        & 5 & (2601, 13.85089) & (941, 5.995754) & (749, 4.323002) & (923, 3.913824) \\
        & 10 & (2606, 17.86887) & (974, 7.244179) & (674, 4.795776) & (967, 4.370866) \\
        & 15 & (2606, 22.462996) & (940, 8.762238) & (677, 5.658468) & (870, 5.10412) \\
        & 20 & (2606, 26.806823) & (960, 10.224163) & (705, 6.411012) & (888, 5.76321) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (2660, 11.641451) & (759, 5.143468) & (635, 3.952877) & (753, 3.644825) \\
        & 5 & (2644, 13.210472) & (866, 5.820045) & (617, 4.187215) & (818, 3.821646) \\
        & 10 & (2601, 17.397328) & (937, 7.049637) & (762, 4.711021) & (867, 4.349421) \\
        & 15 & (2606, 21.439289) & (983, 8.432824) & (705, 5.630066) & (867, 5.113627) \\
        & 20 & (2606, 26.201712) & (951, 10.179697) & (719, 6.563192) & (870, 5.757685) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (2660, 7.014586) & (759, 4.099205) & (507, 3.402992) & (535, 3.265395) \\
        & 2 & (2644, 8.570758) & (866, 4.560648) & (518, 3.426621) & (538, 3.325384) \\
        & 5 & (2601, 11.002977) & (906, 5.279612) & (617, 3.9874) & (564, 3.80108) \\
        & 10 & (2606, 15.256073) & (936, 6.663428) & (682, 4.563828) & (571, 4.192416) \\
        & 15 & (2606, 19.08951) & (954, 7.858194) & (655, 5.383557) & (651, 4.826672) \\
        & 20 & (2606, 23.448812) & (944, 9.089351) & (682, 6.010336) & (622, 5.58813) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (563, 7.180937) & (666, 4.328697) & (606, 3.496552) & (738, 3.371479) \\
        & 2 & (618, 8.639106) & (414, 4.809814) & (689, 3.638419) & (912, 3.561971) \\
        & 5 & (598, 10.839214) & (610, 5.62101) & (772, 4.184578) & (921, 3.808747) \\
        & 10 & (604, 14.174811) & (595, 6.497019) & (796, 4.620337) & (923, 4.280902) \\
        & 15 & (618, 18.288144) & (594, 7.977383) & (807, 5.632297) & (837, 5.012554) \\
        & 20 & (612, 22.374368) & (640, 9.567872) & (807, 6.256049) & (837, 5.788372) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (532, 7.518926) & (371, 4.91902) & (409, 4.087247) & (380, 3.841569) \\
        & 2 & (530, 12.03291) & (287, 6.96289) & (443, 5.47965) & (419, 4.904233) \\
        & 5 & (577, 22.764435) & (300, 12.170004) & (470, 8.886947) & (416, 7.767748) \\
        & 10 & (613, 39.233378) & (332, 21.191422) & (523, 14.484679) & (445, 12.271197) \\
        & 15 & (613, 38.239648) & (359, 18.641235) & (590, 13.312159) & (515, 11.42225) \\
        & 20 & (613, 41.894058) & (411, 19.597006) & (629, 13.746571) & (542, 11.971981) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (219, 2.906677) & (78, 2.720494) & (116, 2.747374) & (184, 2.789192) \\
        & 2 & (219, 3.663202) & (78, 2.963913) & (116, 2.88292) & (184, 2.912347) \\
        & 5 & (219, 5.929757) & (78, 3.733847) & (116, 3.341918) & (184, 3.293982) \\
        & 10 & (316, 9.966511) & (170, 5.009166) & (191, 4.191981) & (346, 3.908425) \\
        & 15 & (219, 13.353948) & (78, 6.313105) & (116, 4.734477) & (184, 4.500818) \\
        & 20 & (219, 17.166411) & (78, 7.551934) & (116, 5.43375) & (184, 5.182752) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (3, 4.93581) & (50, 3.678218) & (-68, 3.118525) & (-2, 3.084485) \\
        & 2 & (9, 5.627936) & (2, 3.963403) & (115, 3.250154) & (54, 3.154718) \\
        & 5 & (6, 7.074868) & (77, 4.426632) & (181, 3.55516) & (271, 3.391911) \\
        & 10 & (27, 11.565817) & (111, 6.226378) & (165, 4.524875) & (335, 4.239357) \\
        & 15 & (17, 14.382752) & (167, 6.908416) & (112, 5.006554) & (282, 4.594821) \\
        & 20 & (52, 19.584597) & (129, 8.378082) & (238, 5.881316) & (348, 5.450063) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{brightkite}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_brightkite}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (511, 4.331406) & (2251, 5.445484) & (2293, 5.092611) & (4206, 5.190955) \\
        & 2 & (511, 7.368159) & (2251, 7.866471) & (2486, 6.35433) & (4054, 6.097935) \\
        & 5 & (544, 9.032235) & (2371, 8.981611) & (2590, 7.032122) & (4067, 6.437749) \\
        & 10 & (526, 11.510036) & (2419, 11.134309) & (2668, 8.266657) & (3971, 6.609456) \\
        & 15 & (552, 15.222338) & (2419, 14.188718) & (2738, 9.63729) & (4320, 7.399298) \\
        & 20 & (556, 18.698971) & (2464, 16.68068) & (2738, 11.13879) & (4326, 7.999017) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (511, 7.321111) & (2251, 7.676253) & (2486, 6.339604) & (4054, 6.03925) \\
        & 5 & (554, 8.473394) & (2260, 8.626599) & (2509, 7.061166) & (4270, 6.04146) \\
        & 10 & (561, 11.800697) & (2391, 11.205999) & (2673, 8.185404) & (3982, 6.583055) \\
        & 15 & (526, 14.552206) & (2419, 13.813283) & (2668, 9.529306) & (4116, 7.424883) \\
        & 20 & (526, 18.264272) & (2419, 16.406695) & (2738, 11.096055) & (4220, 7.607183) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (511, 3.870919) & (2251, 4.976404) & (2293, 4.810573) & (4206, 4.784768) \\
        & 2 & (554, 5.19664) & (2260, 5.952932) & (2587, 5.369132) & (4178, 4.922209) \\
        & 5 & (561, 7.048542) & (2391, 7.489798) & (2736, 5.913927) & (3951, 5.258277) \\
        & 10 & (526, 10.603894) & (2419, 10.044706) & (2696, 7.635753) & (4324, 5.678987) \\
        & 15 & (542, 13.509703) & (2419, 12.478366) & (2696, 8.871025) & (4297, 6.356354) \\
        & 20 & (557, 17.138216) & (2464, 14.813504) & (2803, 10.09049) & (4297, 7.013217) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (253, 3.62462) & (807, 5.110506) & (1941, 5.200724) & (2661, 5.386959) \\
        & 2 & (267, 4.718587) & (838, 5.855962) & (1810, 5.676982) & (3195, 5.39356) \\
        & 5 & (303, 6.34697) & (919, 7.50673) & (1756, 6.367354) & (3077, 5.783836) \\
        & 10 & (298, 8.802689) & (946, 9.613448) & (1975, 7.534384) & (3732, 6.110118) \\
        & 15 & (288, 11.671551) & (953, 11.961914) & (2002, 9.285292) & (3706, 6.872089) \\
        & 20 & (278, 14.307012) & (933, 14.2551) & (2009, 10.585216) & (3873, 7.553795) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (134, 10.738631) & (783, 7.442617) & (1648, 5.438749) & (3330, 4.277926) \\
        & 2 & (142, 18.263571) & (826, 11.940534) & (1749, 7.689251) & (3470, 5.097733) \\
        & 5 & (238, 36.935501) & (895, 21.992599) & (1924, 12.950219) & (3465, 7.417933) \\
        & 10 & (242, 53.261851) & (875, 35.932222) & (1949, 21.180753) & (3888, 11.740368) \\
        & 15 & (242, 58.864717) & (927, 34.930516) & (1959, 19.943574) & (3457, 10.411915) \\
        & 20 & (244, 61.634726) & (928, 37.404548) & (1888, 21.231685) & (3629, 10.944137) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (96, 1.883449) & (333, 2.670745) & (369, 3.156782) & (1273, 3.440137) \\
        & 2 & (96, 2.50555) & (333, 3.098938) & (369, 3.420798) & (1273, 3.596383) \\
        & 5 & (96, 3.918953) & (333, 4.518043) & (369, 4.203173) & (1273, 4.062471) \\
        & 10 & (150, 6.508428) & (473, 6.744301) & (677, 5.571919) & (1337, 4.780549) \\
        & 15 & (96, 9.349192) & (333, 9.112854) & (369, 6.814711) & (1273, 5.572274) \\
        & 20 & (96, 11.92908) & (333, 11.537116) & (369, 8.080567) & (1273, 6.342468) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (2, 2.086758) & (16, 3.947758) & (73, 4.294525) & (218, 4.13741) \\
        & 2 & (7, 2.612672) & (103, 4.312337) & (215, 4.549018) & (1276, 4.31771) \\
        & 5 & (2, 3.625463) & (131, 5.261591) & (594, 5.061123) & (1770, 4.634283) \\
        & 10 & (10, 6.822703) & (300, 8.060247) & (772, 6.506863) & (1994, 5.512082) \\
        & 15 & (12, 9.075867) & (284, 10.132303) & (825, 7.534221) & (2504, 5.927042) \\
        & 20 & (23, 12.33712) & (360, 12.98275) & (845, 9.166356) & (2724, 6.702388) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{enron}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_enron}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (1880, 10.71228) & (3239, 15.911818) & (1202, 13.304726) & (1309, 12.044654) \\
        & 2 & (1880, 19.355977) & (3239, 21.000184) & (1423, 13.881173) & (1154, 12.016041) \\
        & 5 & (1914, 25.084593) & (3210, 24.484485) & (1487, 14.438804) & (1230, 11.795518) \\
        & 10 & (1897, 34.753535) & (3305, 31.267398) & (1668, 14.691768) & (1282, 11.975049) \\
        & 15 & (1897, 46.433482) & (3305, 38.903798) & (1668, 15.861955) & (1419, 12.384224) \\
        & 20 & (1897, 57.769216) & (3305, 45.976823) & (1735, 17.265859) & (1327, 12.78748) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (1880, 18.920002) & (3239, 20.863257) & (1423, 13.529899) & (1154, 11.746036) \\
        & 5 & (1865, 23.131213) & (3239, 23.511837) & (1727, 13.829663) & (1225, 11.902334) \\
        & 10 & (1914, 34.562731) & (3305, 30.660947) & (1670, 14.639725) & (1289, 11.906666) \\
        & 15 & (1897, 43.864536) & (3305, 37.108482) & (1573, 15.868421) & (1247, 12.38159) \\
        & 20 & (1897, 55.831186) & (3305, 45.19937) & (1716, 17.017798) & (1377, 13.189475) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (1880, 9.928412) & (3239, 15.159316) & (1494, 12.704985) & (974, 11.709136) \\
        & 2 & (1865, 14.008636) & (3239, 17.550303) & (1670, 13.081662) & (969, 11.524561) \\
        & 5 & (1914, 20.544462) & (3305, 21.620116) & (1779, 13.34531) & (993, 12.081781) \\
        & 10 & (1897, 31.228379) & (3305, 27.702994) & (1579, 14.490075) & (1037, 11.943175) \\
        & 15 & (1897, 41.566679) & (3305, 34.459385) & (1591, 15.280399) & (1037, 12.185434) \\
        & 20 & (1897, 51.697639) & (3305, 41.698888) & (1678, 16.12399) & (986, 12.690062) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (446, 10.507681) & (1486, 15.723185) & (1202, 13.027482) & (1309, 11.839805) \\
        & 2 & (487, 14.628238) & (1884, 18.08194) & (1472, 13.024111) & (1384, 11.741507) \\
        & 5 & (464, 21.155257) & (1663, 22.202272) & (1597, 13.652119) & (1239, 11.755369) \\
        & 10 & (486, 30.477748) & (1694, 27.723429) & (1651, 14.424961) & (1440, 11.875024) \\
        & 15 & (500, 40.967156) & (2122, 34.057724) & (1651, 15.465994) & (1494, 12.399112) \\
        & 20 & (500, 52.151216) & (1935, 42.542172) & (1797, 16.509463) & (1431, 12.686913) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (185, 15.613714) & (1459, 14.178798) & (1011, 12.249921) & (773, 11.548451) \\
        & 2 & (263, 25.216267) & (1498, 18.081384) & (838, 12.964268) & (776, 11.626199) \\
        & 5 & (374, 49.21995) & (1889, 28.206763) & (1070, 14.966518) & (717, 12.372918) \\
        & 10 & (491, 86.139788) & (2015, 51.823022) & (902, 23.426422) & (967, 17.74904) \\
        & 15 & (463, 88.918728) & (2016, 47.755671) & (1401, 19.107009) & (996, 13.495021) \\
        & 20 & (477, 99.358816) & (2015, 54.490456) & (1352, 19.638155) & (828, 13.64916) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (12, 7.222833) & (0, 10.950282) & (20, 11.108081) & (428, 11.147636) \\
        & 2 & (12, 9.055707) & (0, 12.183232) & (20, 11.29506) & (428, 11.223747) \\
        & 5 & (12, 15.460855) & (0, 15.839832) & (20, 11.986463) & (428, 11.414039) \\
        & 10 & (148, 25.873818) & (138, 22.346785) & (16, 12.837359) & (90, 11.690283) \\
        & 15 & (12, 35.600186) & (0, 29.10255) & (20, 13.885689) & (428, 12.032483) \\
        & 20 & (12, 46.373334) & (0, 34.820893) & (20, 14.854479) & (428, 12.373706) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (0, 8.070257) & (0, 13.770937) & (0, 12.127693) & (88, 11.294168) \\
        & 2 & (7, 9.89358) & (1, 15.024687) & (8, 12.293329) & (96, 11.355414) \\
        & 5 & (1, 13.864795) & (0, 17.633792) & (3, 12.70848) & (273, 11.566043) \\
        & 10 & (13, 26.739019) & (27, 25.426077) & (74, 13.92805) & (174, 11.872816) \\
        & 15 & (25, 34.082305) & (204, 31.451282) & (138, 14.873115) & (401, 12.145065) \\
        & 20 & (22, 46.099643) & (190, 38.863589) & (260, 16.012712) & (440, 12.447638) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{hepph}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_hepph}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (6502, 14.009076) & (7422, 14.679457) & (5780, 16.213886) & (4647, 15.751298) \\
        & 2 & (6502, 22.344013) & (7422, 20.710244) & (6210, 19.447721) & (4934, 16.959438) \\
        & 5 & (6637, 29.08989) & (7533, 25.647605) & (6681, 23.093492) & (5281, 17.980626) \\
        & 10 & (6637, 40.696907) & (7533, 34.454681) & (6437, 26.957407) & (4942, 20.196656) \\
        & 15 & (6637, 52.941491) & (7598, 44.065532) & (6437, 31.977536) & (4901, 22.260134) \\
        & 20 & (6637, 64.841984) & (7598, 53.258305) & (6424, 37.207439) & (4818, 24.122128) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (6502, 22.395535) & (7422, 20.669226) & (6210, 19.259234) & (4934, 17.382814) \\
        & 5 & (6566, 26.95458) & (7383, 24.252107) & (6296, 21.941935) & (4760, 17.675723) \\
        & 10 & (6637, 40.199188) & (7533, 34.247148) & (6258, 26.508954) & (5099, 20.104714) \\
        & 15 & (6637, 50.061666) & (7533, 42.551266) & (6437, 31.300332) & (4868, 22.052029) \\
        & 20 & (6637, 64.309491) & (7598, 53.074237) & (6437, 37.134823) & (5091, 24.256497) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (6502, 13.020298) & (7422, 14.011352) & (5780, 15.102904) & (4647, 15.371281) \\
        & 2 & (6566, 17.572612) & (7383, 17.345369) & (6198, 16.74011) & (4505, 15.681111) \\
        & 5 & (6637, 24.936549) & (7533, 22.787584) & (6498, 20.076558) & (4522, 16.746233) \\
        & 10 & (6637, 36.842822) & (7598, 32.665774) & (6444, 24.675284) & (4522, 18.867458) \\
        & 15 & (6637, 48.663534) & (7598, 41.064545) & (6601, 29.358617) & (4573, 20.916193) \\
        & 20 & (6637, 60.973164) & (7598, 50.015291) & (6512, 34.012869) & (4567, 22.750986) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (724, 12.581297) & (3232, 14.817602) & (5554, 16.286631) & (4633, 16.595315) \\
        & 2 & (724, 16.798537) & (3302, 18.140384) & (5114, 17.774026) & (4654, 16.344556) \\
        & 5 & (731, 23.663116) & (3363, 23.349389) & (5266, 20.962841) & (4906, 17.199864) \\
        & 10 & (733, 33.785853) & (3429, 31.778832) & (5325, 25.200098) & (5058, 19.132696) \\
        & 15 & (739, 46.322793) & (3509, 41.170955) & (5029, 30.604151) & (5198, 22.107354) \\
        & 20 & (730, 56.169985) & (3338, 50.081576) & (5029, 35.782734) & (5165, 23.562279) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (675, 24.167564) & (3003, 20.321986) & (3953, 17.597147) & (4306, 15.468346) \\
        & 2 & (687, 39.750607) & (3061, 30.566673) & (4127, 23.683506) & (4380, 18.519992) \\
        & 5 & (751, 78.414224) & (2945, 55.958911) & (4683, 38.628292) & (4697, 26.570887) \\
        & 10 & (757, 127.379362) & (3214, 93.788406) & (4968, 65.970313) & (4836, 43.972665) \\
        & 15 & (781, 131.775808) & (3350, 93.01329) & (4982, 60.001404) & (4954, 37.727108) \\
        & 20 & (781, 142.780931) & (3180, 102.161783) & (5155, 64.922102) & (4925, 39.824714) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (275, 7.370404) & (874, 10.173047) & (1324, 11.814216) & (491, 12.521565) \\
        & 2 & (275, 9.37843) & (874, 11.923304) & (1324, 12.848376) & (491, 12.910815) \\
        & 5 & (275, 15.794254) & (874, 17.237137) & (1324, 15.893406) & (491, 14.346997) \\
        & 10 & (357, 26.582149) & (1279, 26.279711) & (1653, 21.400361) & (774, 16.745987) \\
        & 15 & (275, 37.006772) & (874, 34.932669) & (1324, 25.826337) & (491, 19.091083) \\
        & 20 & (275, 47.663125) & (874, 43.770436) & (1324, 30.826765) & (491, 21.424672) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (15, 9.700132) & (53, 13.060758) & (251, 14.402305) & (333, 14.10091) \\
        & 2 & (40, 11.891144) & (204, 14.965532) & (870, 15.397589) & (1703, 14.681986) \\
        & 5 & (117, 16.139847) & (850, 18.510415) & (1505, 17.313076) & (2159, 15.575501) \\
        & 10 & (118, 29.474276) & (908, 29.621664) & (1907, 23.615062) & (2917, 18.531446) \\
        & 15 & (139, 37.421587) & (829, 36.361822) & (2366, 27.304857) & (2919, 19.847579) \\
        & 20 & (135, 50.370877) & (1083, 46.770155) & (2524, 32.542717) & (3014, 22.616209) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{epinions}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_epinions}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (1399, 7.953749) & (1806, 7.376449) & (1302, 8.720494) & (1193, 8.159371) \\
        & 2 & (1399, 13.250584) & (1806, 11.222614) & (1859, 10.938343) & (1332, 9.812224) \\
        & 5 & (1404, 16.606493) & (1821, 13.930346) & (1920, 13.012133) & (1400, 11.523038) \\
        & 10 & (1435, 21.827349) & (1872, 18.522814) & (1766, 15.586085) & (1303, 13.396541) \\
        & 15 & (1467, 28.570891) & (1872, 24.503237) & (1574, 20.184689) & (1312, 16.084518) \\
        & 20 & (1467, 34.881025) & (1876, 29.810441) & (1662, 23.744555) & (1326, 18.67953) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (1399, 13.108872) & (1806, 10.868075) & (1859, 10.784598) & (1332, 10.09833) \\
        & 5 & (1407, 15.511006) & (1821, 12.975058) & (1905, 12.289557) & (1279, 11.266874) \\
        & 10 & (1435, 22.817317) & (1834, 18.198366) & (1952, 15.547785) & (1329, 13.307694) \\
        & 15 & (1435, 27.209416) & (1806, 23.174056) & (1820, 19.458249) & (1323, 16.130359) \\
        & 20 & (1445, 35.29857) & (1872, 29.688204) & (1590, 23.624911) & (1336, 18.755269) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (1399, 7.347652) & (1806, 7.081155) & (1728, 7.402999) & (1193, 7.493956) \\
        & 2 & (1407, 9.912281) & (1821, 9.027593) & (1649, 8.69315) & (1224, 8.236692) \\
        & 5 & (1435, 13.420627) & (1821, 12.348087) & (1724, 10.95328) & (1272, 9.71036) \\
        & 10 & (1445, 22.163684) & (1872, 17.916443) & (1645, 14.745402) & (1316, 12.522046) \\
        & 15 & (1467, 25.681819) & (1876, 22.858826) & (1645, 18.432552) & (1324, 14.675866) \\
        & 20 & (1467, 32.023161) & (1876, 28.102126) & (1709, 22.085486) & (1342, 17.1649) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (344, 6.962134) & (734, 7.338649) & (1302, 8.383445) & (1078, 8.590261) \\
        & 2 & (327, 9.15968) & (729, 9.38972) & (1293, 9.778422) & (1198, 9.346424) \\
        & 5 & (373, 12.85268) & (811, 12.347115) & (1361, 11.731662) & (1247, 10.700964) \\
        & 10 & (363, 17.719778) & (742, 16.525877) & (1436, 15.063044) & (1230, 12.823346) \\
        & 15 & (352, 23.680394) & (809, 21.543639) & (1524, 19.290959) & (1133, 16.408843) \\
        & 20 & (354, 29.439376) & (809, 26.545) & (1524, 22.326641) & (1295, 18.101346) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (273, 17.075997) & (608, 12.542701) & (1186, 10.383663) & (974, 9.07537) \\
        & 2 & (264, 29.446356) & (752, 20.999337) & (1090, 16.217407) & (1282, 13.211717) \\
        & 5 & (278, 57.006561) & (774, 41.079849) & (1189, 30.793082) & (1438, 23.824083) \\
        & 10 & (284, 95.389934) & (854, 69.297485) & (1335, 52.808828) & (1500, 41.780687) \\
        & 15 & (284, 93.791758) & (879, 66.696617) & (1377, 50.005423) & (1513, 38.528761) \\
        & 20 & (286, 97.925998) & (880, 71.977105) & (1389, 53.819828) & (1615, 40.939716) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (166, 3.621131) & (533, 4.608468) & (656, 5.246678) & (878, 5.60472) \\
        & 2 & (166, 4.709424) & (533, 5.584783) & (656, 5.87103) & (878, 6.110478) \\
        & 5 & (166, 7.966682) & (533, 8.348632) & (656, 7.968597) & (878, 7.644592) \\
        & 10 & (240, 13.274469) & (557, 13.109462) & (789, 11.400203) & (1073, 10.386018) \\
        & 15 & (166, 18.819954) & (533, 18.035512) & (656, 14.98909) & (878, 12.661607) \\
        & 20 & (166, 24.10867) & (533, 22.786093) & (656, 18.558893) & (878, 15.229757) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (35, 4.760348) & (109, 6.44393) & (108, 7.065213) & (94, 7.287121) \\
        & 2 & (42, 5.93591) & (147, 7.444798) & (305, 7.930402) & (347, 7.920304) \\
        & 5 & (59, 7.972565) & (256, 9.458135) & (514, 9.439179) & (723, 8.825496) \\
        & 10 & (82, 14.790045) & (261, 15.718018) & (653, 13.987663) & (807, 12.326806) \\
        & 15 & (113, 18.800661) & (315, 18.947982) & (658, 16.484998) & (900, 13.760862) \\
        & 20 & (108, 25.363641) & (340, 25.863805) & (566, 20.477926) & (806, 16.893236) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{relato}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_relato}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (18200, 20.066584) & (1525, 10.278747) & (1093, 9.362024) & (732, 8.8609) \\
        & 2 & (18200, 30.911228) & (1631, 10.966134) & (1081, 9.880414) & (601, 8.934576) \\
        & 5 & (17886, 37.100711) & (1769, 11.868651) & (1170, 10.131934) & (727, 9.160244) \\
        & 10 & (17886, 47.582482) & (1815, 12.89966) & (1228, 10.930069) & (724, 9.874507) \\
        & 15 & (17886, 59.291739) & (1634, 14.067592) & (1221, 12.1711) & (737, 10.838254) \\
        & 20 & (17886, 71.037556) & (1634, 15.437461) & (1228, 13.320627) & (756, 11.759433) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (18200, 31.367987) & (1631, 10.950923) & (1081, 9.631465) & (601, 8.898312) \\
        & 5 & (18200, 35.502089) & (1777, 11.500195) & (1111, 10.015313) & (675, 9.169323) \\
        & 10 & (17886, 47.871221) & (1618, 12.671074) & (1259, 10.910955) & (753, 9.767921) \\
        & 15 & (17886, 57.456869) & (1815, 14.061171) & (1236, 11.888506) & (727, 10.982649) \\
        & 20 & (17886, 71.596376) & (1634, 15.462811) & (1236, 12.980841) & (748, 11.536748) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (18200, 18.671986) & (1525, 9.813701) & (860, 9.093311) & (510, 8.63311) \\
        & 2 & (18200, 23.279586) & (1698, 10.157537) & (862, 9.126792) & (537, 8.703942) \\
        & 5 & (17886, 29.692579) & (1514, 10.802643) & (1083, 9.729115) & (570, 9.060151) \\
        & 10 & (17886, 40.454163) & (1508, 12.003224) & (979, 10.872554) & (571, 9.79806) \\
        & 15 & (17886, 52.286336) & (1586, 13.291565) & (1210, 11.522062) & (573, 10.516353) \\
        & 20 & (17886, 62.886783) & (1537, 15.036476) & (1187, 12.597883) & (553, 11.15737) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (3932, 19.492647) & (1398, 10.281061) & (1093, 9.361074) & (732, 8.828502) \\
        & 2 & (3731, 23.300827) & (1554, 10.593149) & (1080, 9.357446) & (770, 9.018518) \\
        & 5 & (3725, 29.477057) & (1542, 11.187701) & (1155, 9.99313) & (798, 9.323371) \\
        & 10 & (3725, 39.646281) & (1567, 12.319004) & (1170, 10.702775) & (738, 9.72672) \\
        & 15 & (3725, 50.968981) & (1443, 13.853482) & (1170, 11.932157) & (788, 10.766915) \\
        & 20 & (3725, 61.487066) & (1499, 15.024706) & (1173, 12.932639) & (802, 11.435084) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (3713, 15.530225) & (1048, 9.655758) & (777, 8.969255) & (495, 8.575624) \\
        & 2 & (3838, 22.892191) & (1259, 11.657735) & (759, 10.429413) & (554, 9.588718) \\
        & 5 & (3906, 42.422152) & (1374, 16.689715) & (717, 13.836441) & (652, 12.155182) \\
        & 10 & (3751, 77.338054) & (1407, 25.30496) & (694, 20.404779) & (697, 17.628668) \\
        & 15 & (3792, 77.208547) & (1445, 23.562442) & (815, 18.741732) & (736, 16.094562) \\
        & 20 & (3792, 88.151785) & (1566, 24.759263) & (746, 19.567629) & (744, 16.827505) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (719, 8.593711) & (610, 7.798539) & (375, 7.781) & (657, 7.841317) \\
        & 2 & (719, 10.628516) & (610, 8.030336) & (375, 7.939821) & (657, 7.975527) \\
        & 5 & (719, 16.820136) & (610, 8.773347) & (375, 8.54328) & (657, 8.386603) \\
        & 10 & (1565, 27.174709) & (823, 9.991018) & (539, 9.470157) & (755, 9.209895) \\
        & 15 & (719, 37.641159) & (610, 11.284551) & (375, 10.396356) & (657, 9.836579) \\
        & 20 & (719, 47.937585) & (610, 12.481733) & (375, 11.305846) & (657, 10.579446) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (26, 13.311316) & (53, 9.054355) & (45, 8.633299) & (56, 8.333059) \\
        & 2 & (133, 15.341061) & (203, 9.317372) & (202, 8.856714) & (109, 8.478147) \\
        & 5 & (1028, 19.566863) & (348, 9.954583) & (347, 9.187858) & (207, 8.818307) \\
        & 10 & (1123, 32.759762) & (403, 11.688949) & (537, 10.80347) & (229, 9.698891) \\
        & 15 & (1417, 40.345749) & (503, 12.404703) & (482, 11.102026) & (282, 10.363468) \\
        & 20 & (879, 52.582941) & (518, 13.748626) & (502, 12.081631) & (336, 11.073083) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{slashdot}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_slashdot}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (3078, 9.137355) & (6872, 23.077852) & (3216, 28.016744) & (1601, 31.364135) \\
        & 2 & (3078, 15.931743) & (6872, 35.356373) & (3216, 34.519191) & (2532, 34.329742) \\
        & 5 & (3078, 22.583234) & (7438, 46.274978) & (3717, 41.788776) & (2658, 39.501804) \\
        & 10 & (2942, 33.817354) & (7410, 67.306994) & (3689, 52.481098) & (3066, 47.082249) \\
        & 15 & (2942, 46.665795) & (7376, 89.841317) & (3760, 66.716082) & (3237, 55.769771) \\
        & 20 & (2942, 57.968247) & (7487, 111.159931) & (3786, 79.026608) & (3260, 66.239228) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (3078, 16.044073) & (6872, 35.108201) & (3216, 33.769681) & (2532, 33.472693) \\
        & 5 & (3078, 20.728486) & (6977, 43.846302) & (3393, 39.830286) & (2466, 37.913488) \\
        & 10 & (2942, 33.712189) & (7387, 65.986137) & (3705, 52.399195) & (3076, 47.011571) \\
        & 15 & (2942, 43.736657) & (7410, 83.202126) & (3877, 64.562998) & (2991, 55.601181) \\
        & 20 & (2942, 57.613948) & (7376, 109.244064) & (3694, 78.403743) & (3278, 66.61477) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (3078, 8.383145) & (6872, 21.465917) & (3216, 26.426679) & (2381, 29.018141) \\
        & 2 & (3078, 13.202961) & (6977, 29.534145) & (3393, 30.959716) & (2445, 31.939913) \\
        & 5 & (2942, 20.100729) & (7387, 41.521061) & (3705, 38.231511) & (2989, 36.817633) \\
        & 10 & (2942, 31.696554) & (7376, 61.768423) & (3694, 51.451934) & (3278, 45.83766) \\
        & 15 & (2942, 44.12425) & (7487, 82.986386) & (3786, 62.135343) & (3260, 53.732327) \\
        & 20 & (2942, 56.538565) & (7487, 104.331364) & (3819, 75.139627) & (3260, 63.18732) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (419, 9.144208) & (2292, 23.211475) & (2594, 27.894258) & (1601, 30.808521) \\
        & 2 & (425, 13.140243) & (2464, 30.368479) & (2583, 31.953489) & (2105, 33.214502) \\
        & 5 & (439, 20.094935) & (2403, 43.179821) & (2345, 38.853809) & (2286, 37.464285) \\
        & 10 & (447, 30.193815) & (2458, 60.519335) & (2342, 50.122045) & (2339, 45.529253) \\
        & 15 & (409, 41.46253) & (2458, 82.493371) & (2373, 64.779021) & (2129, 57.230257) \\
        & 20 & (409, 52.13128) & (2435, 99.477884) & (2252, 76.79444) & (2127, 65.92331) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (365, 25.020149) & (2017, 32.740586) & (2035, 32.208022) & (1695, 32.031095) \\
        & 2 & (380, 41.080853) & (2017, 46.1374) & (2170, 41.072028) & (1874, 38.400952) \\
        & 5 & (391, 81.016286) & (2240, 81.933398) & (2385, 63.984136) & (2047, 55.264581) \\
        & 10 & (391, 133.656234) & (2378, 138.864884) & (2562, 105.211061) & (1881, 88.877944) \\
        & 15 & (412, 136.512992) & (2381, 145.23193) & (2699, 103.561808) & (1920, 84.221371) \\
        & 20 & (415, 147.788968) & (2519, 163.972721) & (2715, 115.110821) & (1935, 92.756394) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (146, 8.032294) & (116, 20.242908) & (142, 23.902179) & (196, 25.865214) \\
        & 2 & (146, 10.182026) & (116, 23.973655) & (142, 26.298077) & (196, 27.51254) \\
        & 5 & (146, 16.575301) & (116, 35.209148) & (142, 33.098032) & (196, 32.672331) \\
        & 10 & (241, 27.0287) & (492, 54.028916) & (581, 45.354465) & (388, 41.016239) \\
        & 15 & (146, 38.067553) & (116, 72.680811) & (142, 55.833599) & (196, 49.720338) \\
        & 20 & (146, 48.803032) & (116, 91.74155) & (142, 67.307069) & (196, 58.03318) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (66, 8.209677) & (99, 21.610461) & (11, 26.46422) & (2, 28.758133) \\
        & 2 & (56, 10.330515) & (121, 25.326023) & (122, 28.75007) & (67, 30.611359) \\
        & 5 & (113, 14.586695) & (243, 32.846758) & (275, 33.366299) & (79, 33.651221) \\
        & 10 & (174, 28.085976) & (332, 57.08309) & (297, 47.721802) & (137, 44.519811) \\
        & 15 & (176, 36.432143) & (385, 70.733631) & (278, 56.186387) & (369, 50.485354) \\
        & 20 & (185, 49.585751) & (625, 94.054384) & (429, 69.665654) & (338, 60.714386) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{syracuse}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_syracuse}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (13584, 42.918833) & (6208, 37.637487) & (4041, 33.792637) & (3162, 31.89478) \\
        & 2 & (13584, 67.972448) & (6208, 46.788955) & (4041, 37.013729) & (3455, 30.918941) \\
        & 5 & (13575, 86.737187) & (6752, 57.790389) & (3823, 39.597373) & (3831, 32.481303) \\
        & 10 & (13599, 119.925492) & (6726, 73.331638) & (4003, 45.031304) & (3831, 34.853393) \\
        & 15 & (13599, 157.43262) & (6609, 92.880868) & (4032, 53.166402) & (3883, 37.619268) \\
        & 20 & (13599, 194.824569) & (6768, 108.651844) & (3854, 59.337779) & (3883, 39.708514) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (13584, 68.083202) & (6208, 46.390997) & (4041, 37.020529) & (3455, 30.987662) \\
        & 5 & (13534, 81.61071) & (6677, 54.475581) & (3832, 39.988916) & (3885, 32.167532) \\
        & 10 & (13575, 119.566966) & (6752, 73.701732) & (3896, 44.986285) & (3831, 34.600187) \\
        & 15 & (13599, 152.357478) & (6707, 87.71731) & (4003, 52.026007) & (4122, 37.404323) \\
        & 20 & (13599, 194.678042) & (6609, 111.009044) & (4032, 58.400001) & (3885, 40.207563) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (13584, 39.784097) & (6208, 35.406014) & (4041, 33.207643) & (3155, 30.838721) \\
        & 2 & (13534, 53.167858) & (6677, 40.995739) & (3832, 33.814285) & (3050, 29.701283) \\
        & 5 & (13575, 73.246415) & (6752, 51.249537) & (3896, 37.390047) & (3634, 31.497672) \\
        & 10 & (13599, 106.95152) & (6609, 68.252545) & (4032, 44.07337) & (3231, 34.835858) \\
        & 15 & (13599, 141.721769) & (6823, 85.316382) & (4032, 49.657822) & (3667, 35.776236) \\
        & 20 & (13599, 177.902717) & (6823, 102.361751) & (3837, 55.366453) & (3667, 38.565606) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (1180, 36.660868) & (1394, 34.937324) & (2062, 34.445082) & (3162, 32.699253) \\
        & 2 & (1475, 49.889538) & (1401, 41.541774) & (2236, 34.817455) & (2604, 31.520299) \\
        & 5 & (1475, 69.707858) & (1732, 51.103882) & (2536, 39.362832) & (3156, 32.904191) \\
        & 10 & (1579, 99.048102) & (1743, 67.193724) & (2516, 43.292258) & (3219, 33.990909) \\
        & 15 & (1556, 137.172782) & (1855, 87.183607) & (2375, 50.947088) & (3754, 37.311674) \\
        & 20 & (1556, 172.371989) & (1698, 104.317272) & (2593, 56.394751) & (3859, 39.280838) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (1577, 47.474689) & (2267, 35.795039) & (2200, 31.486294) & (2080, 28.850227) \\
        & 2 & (2078, 74.812402) & (2283, 47.830792) & (2509, 36.376688) & (2133, 30.553379) \\
        & 5 & (2188, 141.600142) & (2510, 76.865257) & (2699, 48.753152) & (2611, 35.919703) \\
        & 10 & (2188, 230.624679) & (2515, 122.091206) & (2866, 72.79768) & (2667, 50.070531) \\
        & 15 & (2035, 248.787257) & (2583, 127.339392) & (2809, 69.564209) & (2794, 44.51512) \\
        & 20 & (2038, 280.394172) & (2566, 143.537395) & (2907, 74.808112) & (2757, 47.333103) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (329, 21.047036) & (438, 24.928693) & (300, 26.296863) & (176, 26.673974) \\
        & 2 & (329, 28.007259) & (438, 28.143183) & (300, 27.413802) & (176, 27.1633) \\
        & 5 & (329, 45.821058) & (438, 37.908263) & (300, 30.91087) & (176, 28.71001) \\
        & 10 & (574, 78.649986) & (702, 54.212184) & (917, 37.518702) & (439, 31.280486) \\
        & 15 & (329, 110.359272) & (438, 70.787691) & (300, 42.592056) & (176, 34.128857) \\
        & 20 & (329, 139.094946) & (438, 88.008542) & (300, 48.424284) & (176, 36.65451) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (0, 28.390049) & (1, 31.537561) & (116, 30.250711) & (72, 28.421338) \\
        & 2 & (6, 34.359303) & (75, 34.768408) & (9, 31.355581) & (493, 28.907215) \\
        & 5 & (7, 46.523486) & (82, 41.281639) & (557, 33.869331) & (983, 29.929439) \\
        & 10 & (21, 86.319679) & (158, 62.431811) & (428, 40.812047) & (989, 33.312353) \\
        & 15 & (22, 108.426765) & (197, 73.398591) & (418, 44.921136) & (1245, 35.22558) \\
        & 20 & (37, 146.327001) & (333, 92.227997) & (849, 51.733232) & (1628, 37.525779) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{gowalla}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_gowalla}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (2156, 17.250765) & (4639, 34.457268) & (4558, 50.228279) & (3348, 62.148935) \\
        & 2 & (2156, 28.167689) & (4639, 51.946555) & (4558, 68.217324) & (3348, 79.537184) \\
        & 5 & (2169, 39.767643) & (4828, 70.161341) & (4815, 88.415418) & (3600, 95.969509) \\
        & 10 & (2209, 59.279109) & (4991, 104.108203) & (5175, 122.547026) & (4051, 127.31719) \\
        & 15 & (2169, 80.004062) & (4991, 136.618916) & (5372, 159.781998) & (4617, 160.744555) \\
        & 20 & (2181, 101.828541) & (4991, 172.50932) & (5372, 199.099672) & (4652, 189.724944) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (2156, 28.096701) & (4639, 52.097043) & (4558, 68.635538) & (3348, 78.514117) \\
        & 5 & (2169, 36.565866) & (4639, 64.364222) & (4720, 81.717093) & (3480, 90.34128) \\
        & 10 & (2169, 59.696621) & (4656, 102.948816) & (5221, 121.257137) & (3851, 125.697294) \\
        & 15 & (2209, 76.146773) & (4991, 129.479459) & (5175, 152.444814) & (3853, 152.075571) \\
        & 20 & (2241, 99.555031) & (4991, 168.191196) & (5372, 196.499618) & (4051, 188.770842) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (2156, 15.817059) & (4639, 33.14413) & (4558, 48.953266) & (3348, 61.198515) \\
        & 2 & (2169, 23.972167) & (4639, 45.983909) & (4720, 63.230449) & (3480, 73.074145) \\
        & 5 & (2169, 36.35377) & (4656, 65.563888) & (5221, 84.586214) & (3851, 91.057811) \\
        & 10 & (2241, 60.956302) & (4991, 98.907459) & (5372, 121.011317) & (4051, 122.64463) \\
        & 15 & (2173, 77.744099) & (4991, 132.748716) & (5372, 158.346635) & (4652, 154.625164) \\
        & 20 & (2340, 100.499021) & (4991, 168.338879) & (5372, 195.343929) & (4599, 185.53489) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (585, 15.390641) & (1665, 33.078106) & (2011, 49.502759) & (2408, 62.065986) \\
        & 2 & (588, 23.13957) & (1653, 44.773951) & (1850, 62.257377) & (2217, 73.81874) \\
        & 5 & (584, 33.783655) & (1524, 62.245573) & (2022, 82.289333) & (2352, 91.868419) \\
        & 10 & (574, 51.673385) & (1516, 90.121998) & (2173, 113.223071) & (2593, 119.825747) \\
        & 15 & (580, 70.769903) & (1516, 121.838574) & (2169, 145.921236) & (2342, 150.819693) \\
        & 20 & (582, 88.914154) & (1517, 149.250357) & (2095, 177.999262) & (2400, 180.99605) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (476, 58.926643) & (1558, 64.954823) & (1915, 71.927896) & (1748, 77.397144) \\
        & 2 & (545, 99.766209) & (1596, 101.376652) & (2067, 102.452668) & (2105, 100.385736) \\
        & 5 & (589, 200.149661) & (1748, 191.729642) & (2353, 177.370222) & (2209, 159.370979) \\
        & 10 & (589, 334.970778) & (1870, 319.254124) & (2590, 288.175274) & (2651, 250.22854) \\
        & 15 & (603, 325.665102) & (1940, 317.799222) & (2678, 293.884366) & (2481, 256.016475) \\
        & 20 & (607, 346.781807) & (1940, 349.985538) & (2790, 324.063543) & (2600, 285.047393) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (309, 13.788904) & (216, 28.110017) & (190, 43.50338) & (113, 55.991149) \\
        & 2 & (309, 17.40175) & (216, 33.555561) & (190, 49.712142) & (113, 62.696089) \\
        & 5 & (309, 28.33458) & (216, 50.846547) & (190, 68.710448) & (113, 79.404135) \\
        & 10 & (329, 47.057335) & (695, 79.058022) & (434, 102.175082) & (392, 108.591515) \\
        & 15 & (309, 65.575881) & (216, 108.238793) & (190, 132.052858) & (113, 137.83236) \\
        & 20 & (309, 83.175236) & (216, 137.192202) & (190, 163.539437) & (113, 166.78048) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (0, 14.388134) & (0, 31.767857) & (0, 48.771893) & (20, 62.0023) \\
        & 2 & (1, 18.149702) & (5, 37.393978) & (55, 55.114615) & (116, 67.78141) \\
        & 5 & (2, 25.468295) & (12, 48.794362) & (66, 67.796522) & (26, 79.191418) \\
        & 10 & (12, 47.65298) & (19, 85.499047) & (100, 108.456509) & (81, 115.707457) \\
        & 15 & (13, 61.772505) & (46, 105.917868) & (104, 130.881632) & (270, 137.866356) \\
        & 20 & (17, 84.348169) & (32, 140.406237) & (201, 168.625494) & (217, 172.471614) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{twitter}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_twitter}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (5792, 32.22977) & (25273, 32.191346) & (12588, 38.239932) & (1068, 44.567476) \\
        & 2 & (5406, 51.697749) & (25523, 48.436832) & (14172, 52.23859) & (993, 54.257068) \\
        & 5 & (4919, 69.780089) & (25445, 66.888133) & (14820, 68.372353) & (1085, 66.340954) \\
        & 10 & (6309, 105.836748) & (25574, 100.419997) & (14715, 101.620759) & (149189, 100.941726) \\
        & 15 & (7288, 135.667083) & (25574, 132.941585) & (15129, 130.15164) & (149188, 124.15587) \\
        & 20 & (7494, 170.204321) & (25672, 168.079383) & (17087, 165.087614) & (149176, 156.316675) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (5406, 51.869004) & (25523, 48.432708) & (14172, 52.378278) & (993, 54.443817) \\
        & 5 & (6741, 64.559927) & (25445, 60.918173) & (15350, 63.883068) & (1507, 63.765601) \\
        & 10 & (6986, 101.530793) & (26344, 98.349682) & (14347, 101.317042) & (148768, 99.605697) \\
        & 15 & (6992, 129.077426) & (25586, 126.146423) & (14669, 129.259442) & (1929, 107.28004) \\
        & 20 & (7047, 168.380577) & (25586, 166.89998) & (18161, 161.833963) & (2362, 134.152945) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (5792, 30.174098) & (25273, 31.20066) & (12588, 37.185525) & (1887, 43.346764) \\
        & 2 & (5792, 43.317874) & (25453, 43.40582) & (14225, 48.705107) & (2014, 50.856149) \\
        & 5 & (5948, 63.137128) & (25465, 64.157894) & (19593, 65.183179) & (1495, 65.033025) \\
        & 10 & (6385, 96.344019) & (25398, 97.407013) & (22378, 99.228458) & (119139, 88.479309) \\
        & 15 & (6380, 129.943815) & (25692, 133.076064) & (17087, 127.554944) & (1930, 110.292199) \\
        & 20 & (7090, 162.720907) & (25684, 167.108386) & (14767, 158.833008) & (119139, 135.438184) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (4675, 29.207645) & (8406, 31.45901) & (13057, 36.980751) & (1068, 43.652551) \\
        & 2 & (3658, 41.505399) & (20216, 42.844049) & (13337, 47.190616) & (1611, 51.012466) \\
        & 5 & (5096, 59.139864) & (20619, 61.069498) & (14106, 63.702171) & (148768, 69.591456) \\
        & 10 & (5091, 88.221983) & (8406, 91.471204) & (15410, 90.407044) & (149176, 94.918306) \\
        & 15 & (5087, 119.665234) & (20720, 121.399374) & (17017, 117.710842) & (149188, 121.505219) \\
        & 20 & (5264, 150.64538) & (8406, 155.302002) & (16280, 146.199353) & (149190, 147.688692) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (1347, 85.938826) & (2766, 75.619618) & (11628, 66.656098) & (0, 59.299755) \\
        & 2 & (1347, 121.679605) & (1690, 86.804609) & (8219, 82.54612) & (930, 81.934731) \\
        & 5 & (1447, 206.327432) & (3680, 135.998975) & (4050, 110.855094) & (743, 124.472368) \\
        & 10 & (1706, 314.501682) & (6224, 243.396519) & (10790, 230.891864) & (710, 190.639052) \\
        & 15 & (1992, 390.721497) & (6225, 302.550387) & (27415, 267.379108) & (1697, 203.172245) \\
        & 20 & (2121, 417.767729) & (6225, 342.265757) & (10872, 291.925606) & (847, 224.827101) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (18, 23.140345) & (1605, 30.113673) & (15, 35.068699) & (0, 41.998658) \\
        & 2 & (18, 29.351086) & (1605, 36.695096) & (15, 40.527794) & (0, 47.790536) \\
        & 5 & (18, 48.526995) & (1605, 54.255724) & (15, 56.555583) & (0, 60.634051) \\
        & 10 & (649, 80.425189) & (2740, 84.403829) & (15, 82.86777) & (0, 83.096467) \\
        & 15 & (18, 109.869827) & (1605, 114.536891) & (15, 109.623321) & (0, 105.489152) \\
        & 20 & (18, 140.707342) & (1605, 148.581678) & (15, 137.350974) & (0, 127.577672) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (0, 24.450804) & (1, 31.233218) & (-11, 36.223551) & (-48, 41.869068) \\
        & 2 & (0, 30.485499) & (2, 37.26326) & (0, 41.262597) & (25, 45.953401) \\
        & 5 & (0, 42.50117) & (2, 49.479786) & (0, 51.695204) & (0, 54.720054) \\
        & 10 & (1, 80.653146) & (1, 85.758497) & (17, 84.920984) & (9, 82.029572) \\
        & 15 & (0, 102.999965) & (4, 108.338868) & (111, 104.065065) & (62, 98.417199) \\
        & 20 & (1, 139.453087) & (10, 146.111188) & (3, 135.508874) & (25, 124.279489) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{stanford}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_stanford}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (34727, 96.815317) & (13903, 88.077645) & (7313, 79.695829) & (7933, 74.58187) \\
        & 2 & (34727, 163.800204) & (13903, 101.660277) & (7358, 84.292301) & (8619, 75.905248) \\
        & 5 & (35472, 210.667127) & (13712, 116.792159) & (7474, 90.294164) & (8364, 79.933056) \\
        & 10 & (35483, 296.104172) & (13549, 141.735323) & (6773, 101.146874) & (9058, 85.75348) \\
        & 15 & (35483, 379.843322) & (13549, 167.357328) & (6773, 112.453282) & (8655, 92.784557) \\
        & 20 & (35483, 470.990498) & (13549, 193.362098) & (6773, 123.598105) & (8801, 99.734185) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (34727, 162.052522) & (13903, 101.409627) & (7358, 84.475508) & (8619, 75.585538) \\
        & 5 & (35057, 196.236969) & (13650, 112.538271) & (6727, 89.331761) & (8552, 79.23621) \\
        & 10 & (35472, 291.866031) & (13549, 141.026136) & (6823, 100.507107) & (8891, 85.741432) \\
        & 15 & (35483, 363.928129) & (13549, 163.431182) & (6761, 110.469261) & (8861, 91.665476) \\
        & 20 & (35483, 467.948006) & (13549, 193.633128) & (6773, 123.979598) & (8967, 99.959984) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (34727, 91.237944) & (13903, 86.955482) & (7313, 79.52332) & (7933, 74.978634) \\
        & 2 & (35057, 126.056803) & (13650, 96.646623) & (7361, 82.315159) & (8332, 75.345899) \\
        & 5 & (35472, 175.673164) & (13549, 111.462079) & (7773, 89.368702) & (8364, 78.324265) \\
        & 10 & (35483, 259.633478) & (13549, 135.378938) & (7078, 100.353824) & (8260, 86.502816) \\
        & 15 & (35483, 347.251763) & (13549, 164.680759) & (7212, 112.436771) & (8294, 92.507716) \\
        & 20 & (35442, 437.978777) & (13549, 188.161939) & (7212, 123.091461) & (8625, 99.140762) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (5661, 89.014214) & (7077, 84.894401) & (5199, 83.422277) & (8145, 75.072201) \\
        & 2 & (5479, 121.469296) & (7999, 92.596306) & (5880, 82.015747) & (8581, 73.922073) \\
        & 5 & (5502, 167.262149) & (8450, 107.182301) & (5533, 91.749191) & (8682, 78.988132) \\
        & 10 & (5520, 246.015041) & (8261, 129.768289) & (5921, 98.238124) & (8921, 84.525209) \\
        & 15 & (5796, 333.021418) & (8261, 154.97954) & (5878, 113.489638) & (9052, 91.156537) \\
        & 20 & (5796, 413.023137) & (7483, 177.147368) & (6062, 121.723597) & (9059, 98.88832) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (3382, 103.389162) & (5724, 79.779424) & (2916, 74.370836) & (5361, 71.278303) \\
        & 2 & (3859, 151.221716) & (6139, 92.829653) & (3099, 79.956918) & (5771, 72.274644) \\
        & 5 & (4147, 270.213349) & (7012, 123.380309) & (3480, 93.147245) & (5908, 79.698591) \\
        & 10 & (4179, 466.206248) & (7186, 185.257056) & (4242, 127.623758) & (6223, 97.864621) \\
        & 15 & (4418, 517.675057) & (7995, 189.778014) & (4095, 122.447309) & (6103, 93.907214) \\
        & 20 & (4498, 597.433512) & (7995, 216.309984) & (4110, 133.193601) & (6092, 100.494656) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (139, 63.555624) & (595, 70.558657) & (371, 69.325438) & (3312, 68.733193) \\
        & 2 & (139, 79.795067) & (595, 73.237299) & (371, 71.77277) & (3312, 71.158174) \\
        & 5 & (139, 127.806795) & (595, 87.703684) & (371, 78.094574) & (3312, 75.459431) \\
        & 10 & (506, 208.08281) & (1191, 111.561699) & (814, 90.293125) & (4510, 81.541043) \\
        & 15 & (139, 290.510849) & (595, 136.452374) & (371, 99.434331) & (3312, 86.7421) \\
        & 20 & (139, 371.255455) & (595, 161.463131) & (371, 110.222559) & (3312, 96.512952) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (0, 64.169277) & (31, 81.413712) & (11, 76.234492) & (0, 70.665266) \\
        & 2 & (121, 79.942868) & (250, 85.861006) & (545, 78.40747) & (3264, 72.485616) \\
        & 5 & (140, 112.099574) & (462, 95.675977) & (635, 82.484578) & (4441, 75.22764) \\
        & 10 & (37, 210.442689) & (697, 126.084332) & (1648, 95.920044) & (4859, 86.439338) \\
        & 15 & (208, 271.602123) & (727, 141.739601) & (1807, 103.595016) & (4414, 88.147885) \\
        & 20 & (197, 367.440253) & (1038, 172.267636) & (1989, 116.029053) & (4467, 95.818715) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{youtube}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_youtube}
\end{table*}

\begin{table*}[h!]
    \centering
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        algorithm & $n_c$ & $k=5$ & $k=10$ & $k=15$ & $k=20$ \\
        \hline
        \multirow{6}{*}{BM}
        & 1 & (69841, 184.947758) & (15865, 109.131924) & (6154, 125.102625) & (1973, 116.184614) \\
        & 2 & (69841, 269.715721) & (16639, 156.3468) & (6487, 148.578884) & (2187, 136.397296) \\
        & 5 & (70392, 333.232194) & (17250, 188.865752) & (6246, 172.212999) & (2336, 159.929409) \\
        & 10 & (70184, 447.916909) & (17482, 263.394664) & (6246, 217.438621) & (2347, 198.744257) \\
        & 15 & (70184, 559.750126) & (17482, 321.388279) & (5906, 267.584617) & (2299, 226.794706) \\
        & 20 & (70184, 681.211728) & (17482, 392.373696) & (4467, 312.21477) & (2357, 269.380681) \\
        \hline
        \multirow{6}{*}{EQ}
        & 1 & N/A & N/A & N/A & N/A \\
        & 2 & (69841, 270.361965) & (16639, 156.262437) & (6487, 149.014505) & (2187, 135.776025) \\
        & 5 & (70289, 314.912242) & (17348, 175.188496) & (6508, 164.977351) & (2258, 150.627091) \\
        & 10 & (69737, 444.372591) & (17482, 260.021884) & (6246, 215.380874) & (2342, 196.503726) \\
        & 15 & (70184, 534.436413) & (17482, 310.851462) & (6246, 259.94217) & (2269, 222.622928) \\
        & 20 & (70184, 670.27082) & (17482, 388.571692) & (5906, 317.5184) & (2257, 270.485292) \\
        \hline
        \multirow{6}{*}{II}
        & 1 & (69841, 179.602117) & (15865, 108.033626) & (6154, 124.044298) & (1973, 117.409596) \\
        & 2 & (70289, 225.902993) & (16368, 134.849478) & (6237, 140.792145) & (1983, 132.427966) \\
        & 5 & (69737, 285.287187) & (16158, 176.135094) & (6246, 169.299593) & (2217, 152.173485) \\
        & 10 & (70184, 399.478906) & (16168, 246.115413) & (5906, 213.597636) & (2274, 193.611218) \\
        & 15 & (70184, 526.861574) & (16216, 314.135171) & (4467, 258.704611) & (2329, 226.436015) \\
        & 20 & (70184, 642.020926) & (16455, 375.499729) & (4620, 308.995176) & (2280, 262.455593) \\
        \hline
        \multirow{6}{*}{IO}
        & 1 & (2295, 115.656188) & (3453, 119.008855) & (3767, 112.720193) & (2021, 122.897098) \\
        & 2 & (2208, 156.583749) & (3866, 141.172058) & (3597, 130.649717) & (2239, 140.72643) \\
        & 5 & (1885, 217.510045) & (3806, 176.122573) & (3686, 156.575334) & (2248, 162.098473) \\
        & 10 & (1710, 316.557355) & (3614, 232.498359) & (3711, 198.373934) & (2441, 194.604057) \\
        & 15 & (818, 420.451756) & (3561, 293.285089) & (3590, 242.467404) & (2391, 232.632324) \\
        & 20 & (710, 522.844322) & (3934, 349.380345) & (3640, 285.66923) & (2419, 267.734644) \\
        \hline
        \multirow{6}{*}{NT}
        & 1 & (3361, 154.290558) & (3616, 144.460126) & (2800, 137.186695) & (3539, 142.928956) \\
        & 2 & (3271, 233.801483) & (3625, 188.470627) & (2784, 169.520057) & (3677, 168.023174) \\
        & 5 & (3220, 439.065302) & (3811, 298.813281) & (3030, 251.15891) & (3874, 233.807214) \\
        & 10 & (3494, 705.59448) & (3906, 473.593645) & (3109, 375.332806) & (3990, 342.674057) \\
        & 15 & (3783, 804.524135) & (3967, 495.260585) & (3123, 389.246175) & (4078, 351.200492) \\
        & 20 & (4008, 915.755914) & (4093, 554.369119) & (3147, 429.889279) & (4118, 386.540142) \\
        \hline
        \multirow{6}{*}{NE}
        & 1 & (682, 86.673368) & (648, 101.997978) & (1405, 109.180708) & (1452, 118.312682) \\
        & 2 & (682, 106.525254) & (648, 118.811623) & (1405, 117.111967) & (1452, 125.247142) \\
        & 5 & (682, 167.174618) & (648, 152.96458) & (1405, 142.058964) & (1452, 146.397903) \\
        & 10 & (1344, 267.953063) & (947, 215.08867) & (1510, 181.730074) & (1819, 179.622152) \\
        & 15 & (682, 371.214326) & (648, 279.089291) & (1405, 224.449483) & (1452, 216.560952) \\
        & 20 & (682, 470.687674) & (648, 343.055558) & (1405, 265.112105) & (1452, 250.082739) \\
        \hline
        \multirow{6}{*}{RD}
        & 1 & (23, 89.965633) & (16, 102.005447) & (121, 112.442735) & (155, 122.04761) \\
        & 2 & (51, 109.182972) & (366, 116.9455) & (966, 124.456227) & (779, 130.313734) \\
        & 5 & (119, 150.46222) & (453, 142.383985) & (936, 139.941693) & (1387, 145.472471) \\
        & 10 & (105, 275.956563) & (971, 226.873622) & (1564, 196.010391) & (1854, 196.772464) \\
        & 15 & (159, 353.856702) & (996, 262.244178) & (1770, 232.126078) & (2292, 219.906269) \\
        & 20 & (137, 469.818807) & (1264, 337.926391) & (2056, 290.098063) & (2632, 265.957037) \\
        \hline
    \end{tabular}
    \caption{The full results of the main experiments on \textit{wikitalk}.
        For each algorithm, each considered $k$ value, and each $n_c$, we report the performance (left) and the running time (right).}
    \label{tab:main_wikitalk}
\end{table*}
    

